Concurrent Data Structures Made Easy (Extended Version)

Design of an efficient thread-safe concurrent data structure is a balancing act between its implementation complexity and performance. Lock-based concurrent data structures, which are relatively easy to derive from their sequential counterparts and to prove thread-safe, suffer from poor throughput under even light multi-threaded workload. At the same time, lock-free concurrent structures allow for high throughput, but are notoriously difficult to get right and require careful reasoning to formally establish their correctness. We explore a solution to this conundrum based on batch parallelism, an approach for designing concurrent data structures via a simple insight: efficiently processing a batch of a priori known operations in parallel is easier than optimising performance for a stream of arbitrary asynchronous requests. Alas, batch-parallel structures have not seen wide practical adoption due to (i) the inconvenience of having to structure multi-threaded programs to explicitly group operations and (ii) the lack of a systematic methodology to implement batch-parallel structures as simply as lock-based ones. We present OBatcher-an OCaml library that streamlines the design, implementation, and usage of batch-parallel structures. It solves the first challenge (how to use) by suggesting a new lightweight implicit batching design that is built on top of generic asynchronous programming mechanisms. The second challenge (how to implement) is addressed by identifying a family of strategies for converting common sequential structures into efficient batch-parallel ones. We showcase OBatcher with a diverse set of benchmarks. Our evaluation of all the implementations on large asynchronous workloads shows that (a) they consistently outperform the corresponding coarse-grained lock-based implementations and that (b) their throughput scales reasonably with the number of processors.

==> Makefile <==
all: Makefile *.tex *.bib
	rm -f *.pyg
	pdflatex -shell-escape --jobname=paper paper
	bibtex paper -min-crossrefs=5
	pdflatex -shell-escape --jobname=paper paper
	pdflatex -shell-escape --jobname=paper paper

quick: Makefile *.tex *.bib
	rm -f *.pyg
	pdflatex -shell-escape --jobname=paper paper

appendix:
	pdflatex -shell-escape --jobname=appendix "\def\extflag{}\input{paper}"
	bibtex appendix -min-crossrefs=5
	pdflatex -shell-escape --jobname=appendix "\def\extflag{}\input{paper}"
	pdflatex -shell-escape --jobname=appendix "\def\extflag{}\input{paper}"


clean:
	rm -f *.pyg *.aux *.bbl *.blg *.log *.out *.rel paper*.pdf paper.zip	paper.fdb_latexmk paper.fls appendix.pdf

.PHONY: all clean

zip:
	zip paper.zip Makefile *.tex *.bbl mathpartir.sty references.bib *.sty *.cls images/*.tex images/*.pdf diagrams/* data/**/* *.pyg*


==> abstract-icfp.tex <==
%
% 1. Setup
%
Batch parallelism is an approach for designing high-throughput
concurrent data structures via a simple insight: efficiently
processing a batch of \emph{a priori known} operations in parallel is
easier than optimising performance for a stream of arbitrary
asynchronous concurrent requests.
%
% 2. Challenge
%
Despite the appealing simplicity and theoretical efficiency of
batch-parallel structures, their wide practical adoption in concurrent
applications has been hindered by the following two challenges.
%
First, they are difficult to use in common concurrent applications.
%
Second, implementing such structures from scratch requires one to
intertwine sequential logic with dynamic parallelism, making it easy
to introduce bugs.
%
As a result, few implementations of batch-parallel structures are
currently available, and no uniform framework for building,
evaluating, and using them exists to date.

%
% 3. What we have done to address it
%
In this work, we present \tool---a Multicore OCaml library that
streamlines the usage, design, implementation, and testing of
concurrent batch-parallel structures.
%
\tool solves the first challenge (how to use) by implementing the
\emph{implicit batching} technique, made possible by OCaml's new
mechanism of \emph{algebraic effects}.
%
The second challenge (how to implement) is addressed by structuring
\tool as a composition of OCaml functors, which decouple sequential
data structure logic from parallel processing of batches.
%
% This modular design allows one to introduce parallelism
% \emph{gradually}, starting from a sequential thread-safe structure,
% and then implementing different parallel processing strategies by
% elaborating just \emph{one specific function}.
% %
% Finally, \tool comes with a test harness that automates
% linearisability checking.

We showcase \tool with three case studies: two new efficient instances
of a concurrent map in OCaml, based on a skip list and on a B-tree,
%
and a concurrent thread-safe implementation of a Datalog solver.
%
Our evaluation of all the implementations on large asynchronous
workloads shows that (a)~they consistently outperform the
corresponding coarse-grained lock-based implementations---the only
ones available in OCaml to date, and that (b)~their throughput
predictably scales with the number of processors.


% %
% % 4. What we have done
% %
% In this work, we present the design and implementation of \tool: the first library for modular implementation of easy-to-use BPDS.
% %
% \tool is implemented in OCaml 5 (\aka Multicore OCaml), and in this paper we describe how the recently introduced language features (\is{what are they}) are essential for the design of an extensible library for high-performance parallel programming.
% %
% % 5. Why it rocks
% %
% We show how the functional design greatly simplifies the task of developing new BPDSs as well as using them in standard concurrent applications in a transparent way.
% %
% Finally, we report on our experience of implementing and evaluating a number of BPDSs from the literature in \tool, demonstrating their superior throughput compared to conventional fine-grained concurrent asynchronous data structures under standard workloads.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> abstract_old.tex <==
% 1. Setup
%
Batch parallelism is an approach for designing concurrent data structures that allow for high degree of parallelism via a simple insight: processing a batch of known operations in parallel is easier than dealing with the arbitrary asynchrony of incoming concurrent requests.
%
% 2. Challenge
%
However, implementing batch-parallel data structures is challenging as their design intertwines the logic for (a) registering incoming operations and returning their results with (b) processing batches of operations in a way that maximises parallelism.
%
Furthermore, the usage of BPDS is also non-trivial as it requires the programmer structure their application in a way that submits multiple operations in batches rather than one by one.
%
% 3. State of the art
%
While the theoretical properties of BPDS have been studied extensively, few practical implementations of them are available, and no uniform framework for implementing, evaluating, and using such data structures exists to date.

%
% 4. What we have done
%
In this work, we present the design and implementation of \tool: the first library for modular implementation of easy-to-use BPDS.
%
\tool is implemented in OCaml 5 (\aka Multicore OCaml), and in this paper we describe how the recently introduced language features (\is{what are they}) are essential for the design of an extensible library for high-performance parallel programming.
%
% 5. Why it rocks
%
We show how the functional design greatly simplifies the task of developing new BPDSs as well as using them in standard concurrent applications in a transparent way.
%
Finally, we report on our experience of implementing and evaluating a number of BPDSs from the literature in \tool, demonstrating their superior throughput compared to conventional fine-grained concurrent asynchronous data structures under standard workloads.


==> btree.tex <==
\subsection{Batch-Parallel B-Tree}
\label{sec:btree}

Let us now move from the previous pointer-chasing skip list to a
data structure more suitable for the functional palate: a B-tree.
%
In this section, we present the \emph{first batch-parallel}
implementation for a B-tree's standard interface that provides the
\emph{search} and \emph{insert} operations.
%
We describe the new technique to exploit hidden parallelism in B-tree
when processing a batch of operations and demonstrate that this
construction exhibits scalable throughput and outperforms both a
coarse-grained concurrent wrapper over a B-tree and the
sequential implementation.

\subsubsection{The basics of B-trees}

A B-tree is a widely-used tree data structure that can be used to
implement an efficient set or map interface.
%
The B-tree's efficiency arises from the fact that its operations are
carefully structured to always maintain the balance of the tree and
try to preserve a good distribution of values across the tree, thereby
ensuring a logarithmic lookup time.
%
Before delving into the details of our parallel processing algorithm,
let us refresh the reader's memory on how B-trees store ordered data
and how how implement search and insert operations.

\label{sec:b-tree-data}
\begin{wrapfigure}[9]{r}{0.47\linewidth}
\setlength{\belowcaptionskip}{-15pt}
%\setlength{\abovecaptionskip}{5pt}
\vspace{-13pt}
\includegraphics[width=1.0\linewidth]{images/btree.pdf}
\caption{Structure of a B-tree}
\label{fig:btree}
\end{wrapfigure}
%
\autoref{fig:btree} depicts the general structure of a B-tree.
%
The nodes in a B-tree contain 2 components: a sorted sequence of keys
${k_1, \dots, k_n}$ stored in the node, and a sequence of sub-trees
$c_1, \dots c_{n+1}$ corresponding to the node's children; leaf nodes
contain keys, but no children.
%
The B-tree forms a search tree in the fact that the keys in a node
define \emph{intervals} that bound the contents of children: a child
$c_i$ will only contain keys that lie in the range
${k_{i-1} \leq v < k_i}$.
%
Finally, in order to provide a consistent performance,
%
the B-tree enforces the constraint that for any node, all of its
sub-trees must all have the same height (\ie, the tree is balanced),
%
and that every interior node will have a number of keys between
$t - 1$ and $2t - 1$, where $t$, the branching factor, is a global
parameter of the tree, ensuring that values are evenly distributed.


\paragraph{Search} 

Searching a B-tree for a particular value can be done a simple
algorithm: when looking for a value in a sub-tree, first check if the
value exists in the keys stored in the current node, otherwise if the
value cannot be found, recursively visit the appropriate child, if it
exists.

%\vspace{0.2em}
\begin{figure}[t]
\setlength{\belowcaptionskip}{-10pt}
\setlength{\abovecaptionskip}{2pt}
\includegraphics[width=0.9\linewidth]{images/btree-split.pdf}
\caption{Splitting a B-tree node}
\label{fig:btree-split-node}
\end{figure}
%
\paragraph{Insert} Adding new values to a B-tree is 
slightly more challenging, because care must be taken to preserve the
B-tree's invariants as we mutate it.
%
The high-level intuition for an insert is to recursively traverse down
the tree to find the leaf into which to insert the value---but what if
the leaf is already at full capacity (\ie, it contains $2t - 1$ keys)?
%
As it turns out, the key component for implementing a safe insert is a
\emph{splitting} operation: when a particular node in the
data structure has reached full capacity, we can gain additional
capacity while preserving the structure's invariants by splitting the
node into two and adding a new key and child to the node's parent, as
shown in \autoref{fig:btree-split-node}.
%
While splitting requires modifying the parent, we can prevent this
from bubbling up the entire B-tree by maintaining an invariant that
the node being visited during the recursive traversal
%
has \emph{at least one free space}, thus, preemptively splitting a
sub-tree before descending down the tree.
%
In this way, even if inserting a value into a node requires splitting,
we can be guaranteed that \emph{no further splits} higher up in the
tree would be required to restore the B-tree's intrinsic invariants.

As a final note, let us observe here that new invariant, on the
capacity of visited nodes, that is used for the insert operation is
only suitable because we are considering inserting a \emph{single}
value into the B-tree.
%
If we consider operations involving more than one element at a time,
as should be the case with algorithm that operates on batches, we
should expect to generalise it accordingly.
%

\subsubsection{A batch-parallel B-tree}
% \item Batching: general idea, pictures again!
% \item Snippets: \code{bop} and friends.
% Having seen the traditional operations on B-tree, we are ready to
% investigate their corresponding batch-parallel versions which now
% accept batches of requests.
% %
% % How can we 
% How can we exploit parallelism in a B-tree?
%
The fact that tree-like data structures are amenable to parellisation
is an observation that should be quite familiar to any functional
programmer, and, for the most part, the B-tree does not break this
trend.
%
\autoref{fig:btree-def-node} presents the obvious divide-and-conquer
strategy for exploiting parallelism when processing batches of
requests for a B-tree:
%
partition the requests by the corresponding sub-tree they belong to,
and then recursively process the children in parallel.
%
As we will see, the key challenge in constructing a batch-parallel
B-tree is in ensuring that the effects of any mutation are suitably
\emph{localised}, so a recursive decomposition is indeed possible.

%
\begin{wrapfigure}[15]{r}{0.38\linewidth}
\setlength{\belowcaptionskip}{-15pt}
\setlength{\abovecaptionskip}{5pt}
\vspace{-19pt}
  \includegraphics[width=1.0\linewidth]{images/btree-divide.pdf}
  \caption{Batch-parallel B-tree processing}
  \label{fig:btree-def-node}
\end{wrapfigure}
%
\paragraph{Search} 
%
As searches do not mutate the B-tree, implementing a batch-parallel
B-tree search directly follows the strategy in
\autoref{fig:btree-def-node}. When processing a batch of values to be
searched, first dispatch the values that occur at the current node,
partition the remaining values by the children, and recurse on each
sub-tree in parallel.
%
The partitioning of values to sub-trees can be made more efficient if
%
the input batch is sorted, as this means that the arguments to
recursive calls can be represented as interval ranges over the batch
so no new allocations are necessary.

\paragraph{Insert}
%
At a high level, the same divide-and-conquer strategy in
\autoref{fig:btree-def-node} should be applicable to B-tree inserts:
when inserting a batch of values into a B-tree, we can partition the
values by sub-trees and recurse on each child in parallel.
%
The problem with this strategy is in ensuring that the nodes of the
B-tree never become over-full during the inserts, as this causes them
to split, possibly causing a cascade of splits to ``bubble up'',
making them interfere with other parallel operations.

In the sequential case, where we only insert one element at a time,
this behaviour was relatively easy to control: as a single insert can
cause at most one child to split, the algorithm simply preemptively
partitions children to ensure that the node being visited at any
recursive call always has at least one free space to accommodate a
further split of one of its own children.
%
We can adopt this same strategy for the batch-parallel insert,
preemptively splitting children if the number of elements to insert in
a given batch could cause the sub-tree to become full. However, as we
will see, a suitable criteria for batches on which to preemptively
split nodes is somewhat intricate to define.

How can we characterise the capacity of a B-tree node, that is, the
number of elements that it is \emph{safe to insert} without splitting
the node?
%
In general, inserting $n$ elements into a given node can require
splitting up to $n$ children in the worst case, \ie, when each of the
elements falls into a \emph{different} child, each of which itself
needs splitting.
%
If we only look at the contents of a single node, then the maximum
capacity of any node will be at most $t$: this follows from the fact
that the B-tree requires that every node has a number of keys between
$t-1$ and $2t - 1$, so starting from the minimum and encountering $t$
splits would already cause the node hit the maximum number of keys.
%
As the size of an input batch is typically far larger than $t$, a
constant parameter of the tree, this overly-conservative bound would
hamper the parallelism of our batched implementation.
%

\begin{wrapfigure}[10]{r}{0.475\linewidth}
  \begin{minipage}{1.0\linewidth}
\setlength{\abovecaptionskip}{0pt}
\vspace{-15pt}
{\footnotesize    \begin{align*}
      \text{nkeys}(n) = & ~ \text{number of keys in the node $n$} \\
      \text{child}(n,i) = &~ \text{$i^\text{th}$ child of the node $n$} \\
      \text{free}(n)  = &~ 2 t - 1 - \text{nkeys}(n) \\
      \text{cap}(n)  = &~ \begin{cases}
            \text{free}(n)  & \text{$n$ is a leaf} \\
                                \begin{matrix}
            \left(1 + \min_i \text{cap}(\text{child}(n, i))  \right) \times \\
               \text{free}(n)
                                \end{matrix}
                            & \text{otherwise} \\
      \end{cases}
    \end{align*}
}  \end{minipage}
\caption{Capacity of a B-tree}
\label{equation:new-capacity}
\end{wrapfigure}
The key insight in our design is in defining a novel notion of
capacity for a B-tree node that is more precise but still relatively
cheap to compute.
%
%
The formal description of our capacity function is presented on the
right.
%
The intuition for the equation is as follows: for a leaf node, the
capacity is simply the number of elements that can be inserted before
it hits max capacity. For an interior node, notice that each time one
of its children splits, it increases the number of keys that the node
has by 1, until it reaches max-capacity at which point an additional
element could cause the node to require splitting.
%
As such, we can conservatively bound the capacity of a node by the
capacity of its children plus 1, that is, the minimum number of
elements to cause a child to split, multiplied by the free slots it
has, the number of times it can allow its children to split.
%
By using the minimum here, we lose some precision in our bound, but
this also means that the value of this statistic can be computed
without imposing significant overhead.
%

Using this new definition of capacity, we can construct a
batch-parallel B-tree insert using the divide-and-conquer strategy
from~\autoref{fig:btree-def-node}.
%
In particular, after partitioning the batches by the children, if the
size of a batch exceeds the capacity for the sub-tree, then we
preemptively split the sub-tree until the desired capacity is reached.
%
Once all the splits have been performed, we can then recursively
insert into the children in parallel, returning to the standard divide
and conquer strategy.
%
Finally, we can use the same technique of sorting the input requests
that we used in the case of search operations to again avoid
allocations during partitioning.


\begin{wrapfigure}[7]{r}{0.35\textwidth}
\vspace{-1.75em}
\begin{minipage}{1.0\linewidth}
\begin{minted}[fontsize=\footnotesize,bgcolor=lgray]{ocaml}
let run_batch t pool ops =
  let searches, inserts = 
     (* partition batch *) in
  sort pool searches; 
  sort pool inserts;
  par_search t pool searches;
  par_insert t pool inserts
\end{minted}
\end{minipage}
\end{wrapfigure}
%
Putting it all together, we incorporate both these search and insert
implementations to instantiate the explicitly batched interface of
\tool and construct an efficient batch-parallel B-tree (right).
%
We first partition the input batch, splitting out the searches and
inserts to be handled separately.
%
These partitions are then pre-sorted using an off-the-shelf parallel
merge-sort implementation.
%
Finally, we execute the requested batch by first dispatching the
searches using our batch-parallel search implementation, and then
subsequently dispatching the inserts using the corresponding
batch-parallel insert one.

\subsubsection{Experiments}
We now make the case for the practical utility of batched B-trees.
% 
While our batch-parallel design allows for parallelism, it does not
necessarily lead to a useful data structure:
%
if overhead imposed by book-keeping for the parallel operations and
\tool's implicit batching is too expensive, then it could be possible
that the batched B-tree performs worse than a simple coarse-grained
implementation.
%
To address this concern, we test our batched B-tree by conducting a
thorough performance evaluation against other implementations of
thread-safe map data structures.

Our experimental setup is as follows: we compare the thread-safe
batched B-tree constructed by \tool against 
%
two coarse-grained wrappers, one over vanilla B-trees and
%
the other over the OCaml's standard library's \code{Map}
data structure.
%
We fix 6 as the branching factor of all B-trees.
%
For each data structure,
%
we initialise it with 2,000,000 randomly generated elements
%
and then evaluate its throughput under a workload of 1,000,000
additional concurrent operations,
%
varying the number of domains used in the program and taking the
average of 5 runs for each configuration.
%
We incorporate the effect of different workload by also varying the
distribution of \emph{searches} and \emph{inserts}, considering four
different settings: one workload of only inserts, one workload of only
searches, one workload with a 90/10 split between searches and
inserts, and finally a workload with an equal 50/50 split between the
operations.

\begin{figure}[t]
  \centering
\input{diagrams/btree-plot}
\caption{Comparison of \tool's B-tree versus other concurrent data structures}
\label{fig:btree-perf-results}
\end{figure}

\autoref{fig:btree-perf-results} presents the results of our
evaluation, and demonstrates the effectiveness of batched B-trees.
%
As the number of domains in the program increases, we see the
throughput of the coarse-grained implementations generally decrease as
the cost of lock contention begins to dominate the execution.
%
In contrast, the batched B-tree is able to better exploit parallelism,
and so we see that once the number of cores exceeds 4, not only does
the batched data structure consistently outperform the coarse-grained
ones, its throughput even increases with the number of domains.
%
Furthermore, for certain workloads, we see that the impact of the
parallelism of the batched implementation is significant enough that
the throughput even exceeds the sequential implementation, in which a
stream of searches/insert operations is performed in a single thread
with no locking whatsoever.

% although
% the comparison here is not as clear, as the behaviour of the
% sequential implementation can be highly dependant on the ordering of
% requests, which cannot be controlled in the concurrent setting.

The reader may have noticed that the performance of the batched B-tree
stabilises at around 6 domains, the branching factor used in the
experiments---as it turns out, this relates to an interesting question
of the choice of data structure parameters.
%
As the branching factor represents the minimum number of children of
the nodes in the tree, below 6 domains, the implementation is unable
to exploit parallelism as effectively as the batched implementations
will consistently spawn more tasks than can be handled by the
available domains when visiting nodes.
%
While larger choices of branching factor could allow for more
parallelism, they also lead to shallower trees, increasing the
quantity of data that would have to be stored before performance
improvements are seen.
%
While we found our choice of branching factor to be suitable for the
workloads we consider in our evaluation, users may obtain even greater
throughput by tuning the B-tree parameters for their use-cases.



% will add once experiments done

% \item Experiments


% \todo{Follow the structure from \autoref{sec:skiplist}. Don't forget about images!}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> datalog.tex <==

\subsection{A Concurrent Datalog Solver}
\label{sec:datalog}

%
While our previous case studies evaluated the utility of \tool \wrt
constructing sorely-needed thread-safe container data structures for
the OCaml ecosystem, they also may have obscured the main strengths of
\tool, which truly lies in the simplicity of its interface allowing it
to be applied to a vast variety of domains.
%
For our final case-study, we demonstrate the generality of \tool by
investigating its use for constructing a \emph{thread-safe} and
\emph{efficient} wrapper over a popular OCaml Datalog library with
minimal additional implementation effort.

\subsubsection{A sequential Datalog solver}
\begin{wrapfigure}[8]{r}{0.3\textwidth}
\vspace{-2.0em}
\begin{minipage}{1.0\linewidth}
\begin{minted}[fontsize=\footnotesize,bgcolor=lgray]{ocaml}
module Datalog : sig
  type db
  type term 

  val insert: 
    db -> term -> unit
  val query: 
    db -> term -> term list
end
\end{minted}
\end{minipage}
\end{wrapfigure}
The library we will be using for our experiments is the
\code{datalog}\footnote{\url{https://github.com/c-cube/datalog}, last
  accessed on 27 February 2023.} development, which provides an
efficient sequential implementation of a Datalog engine in OCaml.
%
The main interface to the library is through a type \code{db} encoding
Datalog databases which can then be manipulated through an imperative
query and insert API as presented on the right.
%
Here, each database \code{db} represents a collection of facts known
to be true, where each fact is a relation applied to zero or more
symbols, \ie, \code{edge("a","b")} might encode knowledge that an edge
exists between nodes \code{"a"} and \code{"b"} in some graph.
%
% For the purposes of our exposition, 
We now briefly describe how the query and insert interface of
\code{datalog} interact with databases.

\paragraph{Insert}
Users can extend a database using the \code{insert} operation,
submitting new facts or adding deductive rules that describe how to
deduce new facts from existing ones.
%
In particular, each deduction rule, \ie, \code{connected(x,y) :- edge(x,y)},
consists of a conclusion, \code{connected(x,y)},
represented as relation applied to symbols or variables, and one or
more premises, \code{edge(x,y)}, encoded similarly, and inform the
database that any occurrence of facts matching the premises should
cause the conclusion to be present.
%
For example, a user might submit the \code{connected} rule above as
part of a larger set of rules to encode connectedness in a graph in
their Datalog database.
%
As an implementation detail, the engine implemented in \code{datalog}
is a bottom-up one, which means that when a new fact or clause is
added to the database, the engine will eagerly compute all new
implications as a result of the inserted value.
%
This is relevant for our purposes because it means that queries in
this framework do not need to mutate the database.

\paragraph{Query}
%
% Once a database has been constructed, the other main interface for
% interacting with it is through the \code{query} function.
%
Once a database has been constructed, \code{datalog} allows users to
query the set of facts in the database using a \code{query}
function.
%
By submitting terms to this function, \ie, \code{edge("a","b")} or
\code{connected("x",y)}, the database will return a list of all facts
that match the query, answering questions such as \emph{is there an
  \code{edge} between \code{"a"} and \code{"b"}?} or \emph{what nodes
  are connected to \code{"x"}?} 
%
Internally, each database computes the matching facts for a query
using an index data structure that is kept updated during inserts, so
queries do not have to mutate the underlying database---a fact that we
can exploit if we implement a {batch-parallel} wrapper for
\code{datalog}.

\subsubsection{A batch-parallel Datalog solver}
The key observation powering our wrapper is that while the
\code{datalog} library's \code{db} type is not thread-safe, it can
easily implement a batch-parallel interface.
%
The \code{datalog} library, much like the vast majority of OCaml code
currently in the ecosystem, was not written with a multicore
environment in mind.
%
The library makes pervasive use of mutation and shared state that
would be challenging to port to a fine-grained implementation.
%
In contrast, implementing a batched interface to the library is
comparatively simple: when handling a batch of requests, as queries do
not mutate the database, dispatch all of them in parallel, and then
evaluate each of the inserts on the database sequentially.
%
We use this simple idea to instantiate \tool's interface with the
\code{datalog} library and construct a new thread-safe Datalog
implementation.

\subsubsection{Experiments}
\begin{wrapfigure}[12]{r}{0.45\textwidth}
\vspace{-3pt}
\setlength{\belowcaptionskip}{-15pt}
\setlength{\abovecaptionskip}{7pt}
\begin{minipage}{1.0\linewidth}
\input{diagrams/datalog-plot.tex}
\end{minipage}
\caption{Comparison of Datalog solvers}
\label{fig:datalog-coarse-grained-results}
\end{wrapfigure}
We evaluate the performance of our construction on a realistic
workload and compare it to other thread-safe wrappers of the
\code{datalog} library.
%
For our experiments, we implement a typical graph-connectedness
constraint system on top of the Datalog database, using a graph of 200
nodes, with 30,000 initial edges, and submit requests that either add
new edges or query about the connectedness of two nodes in the graph.
%
All implementations are evaluated on a workload of 50,000 concurrent
requests, using a standard 90/10 split between queries and inserts,
varying the number of domains and taking the average of 10 runs for
each configuration.
%


\autoref{fig:datalog-coarse-grained-results} presents the results of
this evaluation.
%
As can be seen, our construction is efficient and scales gracefully as
the number of domains increases, while the corresponding
coarse-grained wrapper's performance, following the trends we've seen
before, gradually degrades as more domains are added as it suffers
from increasing lock contention.
%
As an additional reference, our plot also includes the throughput of a
na\"{i}ve batch-parallel implementation of a \code{datalog} wrapper,
which simply executes all operations, queries and inserts alike, in a
sequence.
%
Interestingly, the throughput of this na\"{i}ve implementation still
outperforms the coarse-grained version, showing the benefits of the
amortised cost of locking provided by the batched interface, yet it is
unable to exploit parallelism as well as our full construction, so its
throughput does not increase with the number of domains.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> testing.tex <==
\subsection{Testing a Batch-Parallel Implementation}
\label{sec:testing}
%
While developing batch-parallel data structures may be easier than
their fine-grained counterparts, they are still fundamentally
concurrent algorithms, so ensuring their correctness is not
necessarily an easy task.
%
To ease this pain and help developers gain confidence in their
implementations, \tool also comes with an automated testing harness
for batch-parallel implementations.
%

% \vspace{0.2em}
% \begin{wrapfigure}[9]{r}{0.35\linewidth}
%   \includegraphics[width=1.0\linewidth]{images/testing-diagram.pdf}
%   % \caption{A strategy for batch-parallel testing}
%   % \label{fig:test-batch}
% \end{wrapfigure}

Recall how in~\autoref{sec:ebatcher} we briefly suggested that
reasoning about a batched data structure in terms of
linearisability~\cite{HerlihyW90} also leads to a natural strategy for
their testing.
%
In particular, as the results from executing any batch of requests in
a linearisable implementation must also correspond to some execution
of each of the constituent requests in sequence, we can verify a given
implementation is linearisable by running a batch of requests, and
then checking that a sequential explanation exists.
%
The \tool's testing harness builds on this idea and tests the
batch-parallel implementation by first initialising the data structure
with a sequence of arbitrary operations, and then submits a randomly
generated batch of requests to be executed the \code{run_batch}
function required by our interface.
%
As the requests are submitted to the data structure, the harness
records the results from each interaction.
%
Then, once the execution has completed, the testing framework checks
linearisability by looking, by an exhaustive search of all
permutations, for a sequence of operations that produce the recorded
results.
%
If no such sequence can be found, then the implementation is deemed to
not be linearisable, and an error is raised.

\begin{wrapfigure}[15]{r}{0.475\linewidth}
%\setlength{\belowcaptionskip}{-15pt}
\setlength{\abovecaptionskip}{10pt}
\vspace{-1.75em}
\begin{minipage}{1.0\linewidth}
\begin{minted}[fontsize=\footnotesize,bgcolor=lgray]{ocaml}
let api = [
  val_ "insert" Btree.insert
    (fun resolve key vl -> 
          Mk (Insert (key,vl), resolve))
    (t @-> int @-> int @-> returning unit);

  val_ "search" Btree.search
    (fun resolve key -> 
          Mk (Search key, resolve))
    (t @-> int @-> returning (option int));
]
let init () = Btree.init ()
let () = 
  QCheck.run_tests ~count:100 (init,api)
\end{minted}
\end{minipage}
\caption{Testing B-trees Using \tool}
\label{fig:obatcher-testing-example}
\end{wrapfigure}
%
We have implemented \tool's testing harness as an extension to an
existing property-based testing framework,
\code{multicoretests},\footnote{\url{https://github.com/ocaml-multicore/multicoretests},
  last accessed on 20 February 2023.}
%
inspired by QuickCheck~\cite{ClaessenH00} and published by the
Multicore OCaml developer team for testing concurrent
programs~\cite{ocamlmulticoretest}.
%
To make use of the harness, we provide a modified version of
\code{multicoretests}' specification e-DSL and require developers to
declaratively specify the possible operations on their data type.
%
\autoref{fig:obatcher-testing-example} presents an example of such a
specification for a B-tree data structure (\autoref{sec:btree})
implementing a map-like interface.
%
In the code, the variable \code{api} describes the interface
to the data structure, and records the following four pieces of
information for each operation: 
%
(1) a name for pretty printing
\code{"insert"}, 
%
(2) a value encoding its type
\code{t @-> int @-> int @-> returning unit} for generating inputs,
%
(3) a sequential reference implementation \code{Btree.insert}
that must conform to this type, and finally 
%
(4) a function that constructs the corresponding reified operation for
the interface \code{Mk (Insert (key,vl), resolve)}.
%
Given this specification, the testing harness will then automatically
run a series of random tests as described previously and check that
the data structure's \code{run_batch} function is linearisable.
%
Furthermore, by hooking into \code{multicoretests}'s framework, \tool also
gets shrinking of test-cases for free, so when a linearisability
violation is found, the counterexample is usually of a reasonable size. 

